CHC-COMP 2022: Competition Report

CHC-COMP 2022 is the fifth edition of the competition of solvers for Constrained Horn Clauses. The competition was run in March 2022; the results were presented at the 9th Workshop on Horn Clauses for Verification and Synthesis held in Munich, Germany, on April 3, 2022. This edition featured six solvers, and eight tracks consisting of sets of linear and nonlinear clauses with constraints over linear integer arithmetic, linear real arithmetic, arrays, and algebraic data types. This report provides an overview of the organization behind the competition runs: it includes the technical details of the competition setup as well as presenting the results of the 2022 edition.

==> eptcsdata.tex <==
\providecommand{\firstpage}{44}
\providecommand{\publicationstatus}{G.W. Hamilton, T. Kahsai, M. Proietti (Eds.):\\
Joint International Workshops on \\
Horn Clauses for Verification and Synthesis (HCVS 2022)\\
Verification and Program Transformation (VPT 2022)\\
EPTCS 373, 2022, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.373.5}{10.4204/EPTCS.373.5}}

